Continuous-Time Fixed-Lag Smoothing for LiDAR-Inertial-Camera SLAM

Localization and mapping with heterogeneous multi-sensor fusion have been prevalent in recent years. To adequately fuse multi-modal sensor measurements received at different time instants and different frequencies, we estimate the continuous-time trajectory by fixed-lag smoothing within a factor-graph optimization framework. With the continuous-time formulation, we can query poses at any time instants corresponding to the sensor measurements. To bound the computation complexity of the continuous-time fixed-lag smoother, we maintain temporal and keyframe sliding windows with constant size, and probabilistically marginalize out control points of the trajectory and other states, which allows preserving prior information for future sliding-window optimization. Based on continuous-time fixed-lag smoothing, we design tightly-coupled multi-modal SLAM algorithms with a variety of sensor combinations, like the LiDAR-inertial and LiDAR-inertial-camera SLAM systems, in which online timeoffset calibration is also naturally supported. More importantly, benefiting from the marginalization and our derived analytical Jacobians for optimization, the proposed continuous-time SLAM systems can achieve real-time performance regardless of the high complexity of continuous-time formulation. The proposed multi-modal SLAM systems have been widely evaluated on three public datasets and self-collect datasets. The results demonstrate that the proposed continuous-time SLAM systems can achieve high-accuracy pose estimations and outperform existing state-of-the-art methods. To benefit the research community, we will open source our code at ~\url{https://github.com/APRIL-ZJU/clic}.

==> sections/08_author_bio.tex <==
% \iffalse
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/ljj}}]{Jiajun Lv}
	received the B.Eng. degree in Automation from the Zhejiang University of Technology, in 2018. She is pursuing Ph.D. degree in College of Control Science and Engineering, Zhejiang University, Hangzhou, China, from September, 2018. Her major research interests include sensor calibration, sensor fusion, spatial perception and cognition.
\end{IEEEbiography}
% \vfill
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/Lang}}]{Xiaolei Lang}
	received the B.Eng. degree in Automation from the Zhejiang University of Technology, in 2020. He is currently a master in College of Control Science and Engineering, Zhejiang University, Hangzhou, China. His major research interests include multi-sensor based calibration, odometry and mapping.
\end{IEEEbiography}
% remove spaces https://tex.stackexchange.com/a/524073
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/xu}}]{Jinhong Xu}
    received his MA.Sc degree in Control Science and Engineering from Zhejiang University in 2018. He is currently a researcher in the institute of Cyber Systems and Control, Department of Control Science and Engineering, Zhejiang University. His latest research interests include SLAM, information processing and robotic control. 
\end{IEEEbiography}
% remove spaces https://tex.stackexchange.com/a/524073
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{biography/wmm}}]{Mengmeng Wang} received the B.S. degree and the M.S. degree in control science and engineering from Zhejiang University, Zhejiang, China, in 2015 and 2018, respectively. She is currently working towards the Ph.D degree with the Laboratory of Advanced Perception on Robotics and Intelligent Learning, College of Control Science and Engineering, Zhejiang University. Her research interests include visual tracking, action recognition, computer vision, and deep learning.
\end{IEEEbiography}	
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/Xing}}]{Xingxing Zuo}
	received the B.Eng. degree in Mechanical Engineering from the University of Electronic Science and Technology of China (UESTC), Chengdu, China, in 2016, and the Ph.D. in Control Science and Engineering at Zhejiang University, Hangzhou, China, in 2021. 
	
	He is currently a Postdoc researcher at Technical University of Munich. His research interests include computer vision, state estimation, sensor fusion, deep learning, localization and mapping for autonomous robots in complex environments. Dr. Zuo was the Finalist for the ICRA 2021 Best Paper Award in Robot Vision.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/ProfLiu}}]{Yong Liu}
received the B.S. degree in computer science and engineering and the Ph.D. degree in computer science from Zhejiang University, Hangzhou, China, in 2001 and 2007, respectively.
He is currently a Professor with the Institute of Cyber-Systems and Control, College of Control Science and Engineering, Zhejiang University. His research interests include machine learning, robotics vision, multiple-sensor fusion, and intelligent systems.
\end{IEEEbiography} 
\vfill
